Building Performance Simulations Can Inform IoT Privacy Leaks in Buildings

As IoT devices become cheaper, smaller, and more ubiquitously deployed, they can reveal more information than their intended design and threaten user privacy. Indoor Environmental Quality (IEQ) sensors previously installed for energy savings and indoor health monitoring have emerged as an avenue to infer sensitive occupant information. For example, light sensors are a known conduit for inspecting room occupancy status with motion-sensitive lights. Light signals can also infer sensitive data such as occupant identity and digital screen information. To limit sensor overreach, we explore the selection of sensor placements as a methodology. Specifically, in this proof-of-concept exploration, we demonstrate the potential of physics-based simulation models to quantify the minimal number of positions necessary to capture sensitive inferences. We show how a single well-placed sensor can be sufficient in specific building contexts to holistically capture its environmental states and how additional well-placed sensors can contribute to more granular inferences. We contribute a device-agnostic and building-adaptive workflow to respectfully capture inferable occupant activity and elaborate on the implications of incorporating building simulations into sensing schemes in the real world.

==> vd_0.01.tex <==
\begin{figure}[!htp]
    \begin{tabular}{cccc}
    \subfloat[Bed Door $90^{\circ}$, Bath door $90^{\circ}$ (open-door scenario)]{\includegraphics[width = 0.22\linewidth]{img/vd_0.01/0.jpg}\label{subfig:a}} &
    \subfloat[Bed Door $45^{\circ}$, Bath door $90^{\circ}$]{\includegraphics[width = 0.22\linewidth]{img/vd_0.01/1.jpg}\label{subfig:b}} &
    \subfloat[Bed Door $0^{\circ}$, Bath door $90^{\circ}$]{\includegraphics[width = 0.22\linewidth]{img/vd_0.01/2.jpg}\label{subfig:c}} &
    \subfloat[Bed Door $90^{\circ}$, Bath door $45^{\circ}$]{\includegraphics[width = 0.22\linewidth]{img/vd_0.01/3.jpg}\label{subfig:d}} \\
    \subfloat[Bed Door $45^{\circ}$, Bath door $45^{\circ}$]{\includegraphics[width = 0.22\linewidth]{img/vd_0.01/4.jpg}\label{subfig:e}} &
    \subfloat[Bed Door $0^{\circ}$, Bath door $45^{\circ}$]{\includegraphics[width = 0.22\linewidth]{img/vd_0.01/5.jpg}\label{subfig:f}} &
    \subfloat[Bed Door $90^{\circ}$, Bath door $0^{\circ}$]{\includegraphics[width = 0.22\linewidth]{img/vd_0.01/6.jpg}\label{subfig:g}} &
    \subfloat[Bed Door $45^{\circ}$, Bath door $0^{\circ}$]{\includegraphics[width = 0.22\linewidth]{img/vd_0.01/7.jpg}\label{subfig:h}} \\
    \subfloat[Bed Door $0^{\circ}$, Bath door $0^{\circ}$]{\includegraphics[width = 0.22\linewidth]{img/vd_0.01/8.jpg}\label{subfig:i}} &
    \subfloat[Aggregate latent variable privacy $\text{D}_{0.01}$]{\includegraphics[width = 0.22\linewidth]{img/vd_0.01/combined.jpg}\label{subfig:total}} &
    \subfloat[One light sensor can sense all 64 light states for the open-door scenario using GSCA]{\includegraphics[width = 0.22\linewidth]{img/open_door_0.01.jpg} \label{subfig:GSCA-light}}  &
    % \subfloat[Building Layout]{\includegraphics[width = 0.22\linewidth]{img/210712_copeley_plan.png}} &
    \subfloat[31 sensors are needed to sense a total of 567 states using GSCA for the dynamic-door scenario]{\includegraphics[width = 0.22\linewidth]{img/dynamic_door_0.01.jpg} \label{subfig:GSCA-door}} \\
    \end{tabular}
    \caption{Compilation of the distinctness score $\text{\textbf{D}}_{0.01}$ heat maps for each building configuration. In addition to the resolution of the sensor, the building's physical configuration can also systemically alter inferable states of the sensor set.}
    \label{fig:sims_tau0.01}
\end{figure}
